Tensor-Network-Based Distributed Quantum Dynamics on Independent Quantum Computers

We present an approach based on tensor networks for distributed quantum computing simulation of chemical wavepacket dynamics in a continuous variable representation. The central idea is that the tensor-network representation of the multidimensional time-evolution operator naturally induces an elevated Hilbert space where the dynamics decomposes into a set of independent lower-dimensional propagations. This transformation converts an entangled quantum evolution into a set of parallel computational tasks that can be executed asynchronously across heterogeneous quantum and classical computing architectures. The resulting formalism establishes a direct connection between tensor-network decompositions, uniformly controlled quantum circuits, and asynchronous distributed quantum computing. The approach is developed with a goal towards hybrid quantum/classical implementation, and is appropriate for a general heterogeneous mixture of quantum hardware systems. The experimental realization of the asynchronously distributed quantum processes that arise from the tensor-network decomposition are carried out on the Sandia National Laboratories' trapped-ion quantum computer, where the circuits are compiled using native partial-entangling $XX(\theta)$ gates, reducing the expected two-qubit gate infidelity by more than 30\% relative to conventional fully entangling decompositions. We demonstrate the methodology by quantum computing the vibrational spectra of a small protonated water cluster that shows critical quantum nuclear behavior. Such water cluster systems have been found to be challenging for experimental action spectroscopy and for theory, and here, for the first time, we provide results for vibrational spectroscopy that are in agreement with the respective classical results to within 4cm$^{-1}$, thus allowing for the potential for spectroscopic accuracy from quantum computations.

==> Fig_RzCXRzCXRzCXRzCX.tex <==
        $
        \begin{quantikz}
        \lstick{} & \qw & \qw & \qw & \ctrl{2} & \qw & \qw & \qw & \ctrl{2} & \qw \\
        \lstick{} & \qw & \ctrl{1} & \qw & \qw & \qw & \ctrl{1} & \qw & \qw & \qw \\
        \lstick{} & \gate{R_Z(\theta_0)} & \targ{} & \gate{R_Z(\theta_1)} & \targ{} & \gate{R_Z(\theta_2)} & \targ{} & \gate{R_Z(\theta_3)} & \targ{} & \qw \\
        \end{quantikz}
        $

==> Fig_UDU.tex <==
        $
        \begin{quantikz}
        \lstick{} & \gate[wires=2][1.5cm]{U(t_i)} & \gate[wires=3][1.5cm]{D(t_i)} & \gate[wires=2][1.5cm]{V(t_i)} & \qw \\
        \lstick{} & & & & \qw \\
        \lstick{} & \qw & & \gate{H} & \qw \\
        \end{quantikz}
        $ 

==> Figures/Figure_UCG_TN_1.tex <==
%\begin{figure}[tbp]
%\centering
\begin{quantikz}[row sep={0.6cm}, column sep={0.5cm}]
\lstick{} & \ctrl{2} & \qw \\[-0.3cm]
\midstick{$\hspace{-6mm}\raisebox{-15pt}{$\ket{\beta}$}$} \\
\lstick{} & \ctrl{1} & \qw \\
\lstick{$\ket{\chi}$} & \gate{\mathcal{U}_{\beta}} & \qw
\end{quantikz}
%\caption{Uniformly controlled gate with two control qubits encoding $\beta$.}
%\end{figure}

==> Figures/matrix_3D_beta2_2.tex <==
\[
\hat{U} =
\begin{bmatrix}
\mathcal{U}^{[1]}_{11} \otimes \mathcal{U}^{[2]}_{11} \otimes \cdots \otimes \mathcal{U}^{[N]}_{11} & 0 & 0 & 0 \\[6pt]

0 & \mathcal{U}^{[1]}_{12} \otimes \mathcal{U}^{[2]}_{12} \otimes \cdots \otimes \mathcal{U}^{[N]}_{12} & 0 & 0 \\[6pt]

0 & 0 & \mathcal{U}^{[1]}_{21} \otimes \mathcal{U}^{[2]}_{21} \otimes \cdots \otimes \mathcal{U}^{[N]}_{21} & 0 \\[6pt]

0 & 0 & 0 & \mathcal{U}^{[1]}_{22} \otimes \mathcal{U}^{[2]}_{22} \otimes \cdots \otimes \mathcal{U}^{[N]}_{22}
\end{bmatrix}
\]
